Automated SELinux RBAC Policy Verification Using SMT

Security-Enhanced Linux (SELinux) is a Linux kernel module that allows for a role-based access control (RBAC) mechanism. It provides a fine-grained security framework enabling system administrators to define security policies at the system and application level. Whilst SELinux offers robust security features through a customisable, powerful RBAC model, its manual policy management is prone to error, leaving the system vulnerable to accidental misconfigurations or loopholes. We present a tool to automate the conversion of SELinux policies into satisfiability modulo theories (SMT), enabling the verification of the intended security configurations using automated theorem proving. Our tool is capable of flagging common policy misconfigurations by asserting consistency between supplied RBAC policies and the intended specification by the user in SMT. RBAC policies are inherently complicated to verify entirely. We envision that the automated tool presented here can be further extended to identify an even broader range of policy misconfigurations, relieving the burden of managing convoluted policies on system administrators.

==> chart.tex <==
\begin{figure}[ht]
    \centering
    \begin{small}
    \begin{tikzpicture}
        [node distance=2.2cm, node/.style={draw, text centered, minimum height=0.6cm, rounded corners, fill=blue!20}, >=stealth]
        % Yellow rectangle for the tool
        \fill[yellow!40!white, rounded corners] (1.36,0.5) rectangle (10.22,3.5);
        \node at (9.5,1) {\textbf{Tool}};

        % Flow chart nodes
        \node[node] at (0,2) (user) {User};
        \node[node, right of=user] (libsepol) {\texttt{libsepol}};
        \node[node, right of=libsepol] (modelrs) {\texttt{model.rs}};
        \node[node, right of=modelrs] (pyrs) {\texttt{py.rs}};
        \node[node, right of=pyrs, node distance=2.6cm] (concat) {Concatenator};
        \node[node, right of=concat, node distance=2.6cm] (python) {Python};
        \node[node, right of=python, node distance=1.4cm] (z3) {Z3};

        % Arrows
        \path[->] (user) edge node[midway, below, text width=1cm, align=center] {Policy file} (libsepol);
        \path[->] (libsepol) edge node[midway, below, text width=1cm, align=center] {C policy struct} (modelrs);
        \path[->] (modelrs) edge node[midway, below, text width=1cm, align=center]{Rust policy struct} (pyrs);
        \path[->] (pyrs) edge node[midway, below, text width=1cm, align=center] {Python code} (concat);
        \path[->] (concat) edge node[midway, below, text width=1cm, align=center] {Python code} (python);
        \draw (user) edge[bend left=20,->] node[above] {Additional constraints} (concat);
        \path[->] (python) edge [bend left=30] (z3);
        \path[->] (z3) edge [bend left=30] (python);
    \end{tikzpicture}
    \end{small}
    \vspace{-0.5cm}
    \caption{Overall Flow Structure of the Automation}
    \label{fig-impl}
\end{figure}

